Best of Both Worlds Model Selection

We study the problem of model selection in bandit scenarios in the presence of nested policy classes, with the goal of obtaining simultaneous adversarial and stochastic ("best of both worlds") high-probability regret guarantees. Our approach requires that each base learner comes with a candidate regret bound that may or may not hold, while our meta algorithm plays each base learner according to a schedule that keeps the base learner's candidate regret bounds balanced until they are detected to violate their guarantees. We develop careful mis-specification tests specifically designed to blend the above model selection criterion with the ability to leverage the (potentially benign) nature of the environment. We recover the model selection guarantees of the CORRAL algorithm for adversarial environments, but with the additional benefit of achieving high probability regret bounds, specifically in the case of nested adversarial linear bandits. More importantly, our model selection results also hold simultaneously in stochastic environments under gap assumptions. These are the first theoretical results that achieve best of both world (stochastic and adversarial) guarantees while performing model selection in (linear) bandit scenarios.

==> best_of_both_worlds.tex <==

In this section, we present our algorithm for adversarial model selection that preserves a logarithmic regret guarantee in case it interacts with a stochastic environment with a gap. Recall from \pref{sec:setup} that a gap $\Delta$ exists if there exists a unique optimal policy $\pi^* \in \Pi_M$ among all policies $\Pi_M$ such that the expected value of any other policy $\Pi_M \backslash \{ \pi^*\}$ is at least $\Delta$ away from the value of $\pi^*$.

In order to achieve such a best of both worlds guarantee we will combine our adversarial regret balancing technique with the algorithmic strategy of \citet{bubeck2012best}.  The main result for our algorithm is the following:

\begin{theorem}
Consider \pref{alg:gap_estimation_balanced} with inputs $t_0 = 0$, $\wh \pi \in \Pi_M$ arbitrary and $M$ base learners $\alg[1], \dots, \alg[M]$. Then with probability at least $1 - \operatorname{poly}(M)\delta$, the following two conditions hold for all $t \geq M^2$ simultaneously:
 In any adversarial or stochastic environment, the regret is bounded as $\regret(t, \Pi_M) \leq \pref{eqn:arbe_regret} \cdot \sqrt{\log(t+1)}$.
Further, if the environment $\bbB$ is stochastic and there is a unique optimal policy with a gap $\Delta$, then the pseudo-regret is bounded as
    \begin{equation*}
    \pseudoregret(t, \Pi_M) = \widetilde\Ocal\left(  \frac{MR^2(\Pi_M)}{\Delta} \ln(t)\ln \frac{t}{\delta} + \frac{M^4 R^4(\Pi_M) }{R^2(\widetilde \Pi_1) \Delta}  \sqrt{\ln\frac{1}{\delta} \ln\frac{1}{  \Delta}}\ln \frac{t}{\delta}   \right). 
\end{equation*}
Here, $\tilde \Pi_i$ is the extended version of policy class $\Pi_i$ with $(M+1-i)$ additional actions and $i_\star$ the smallest index of the base algorithm that is $h$-stable. 
The $\widetilde \Ocal$-notation omits polynomial factors in $\ln\ln \frac{1}{\delta}, \ln\ln t, \ln M$ and $\ln R(\widetilde \Pi_{M})$.
\end{theorem}

The algorithm has the same regret bound as \textsf{Arbe} up to a $\sqrt{\ln t}$ factor. However, in addition, it also maintains poly-logarithmic pseudo-regret if the environment is stochastic and the best policy exhibits a positive gap. Our pseudo-regret bound depends polynomially on $R(\Pi_M)$ in contrast to the $R(\Pi_{i_\star})$ dependency for the adversarial regret rate. This may seem undesirable but one can show that model selection in stochastic environments with $\poly(R(\Pi_{i_\star}), \ln(R(\Pi_M)) \frac{\ln (t)}{\Delta}$ regret is impossible (see \pref{app:lower_bound}), let alone while maintaining a best-of-both-worlds guarantee with $\sqrt{T}$ regret in adversarial environments. Hence, our algorithm achieves the best kind of guarantee we can hope for, up to improvements in the order of polynomial dependencies.

Our algorithm proceeds in two distinct phases. The first, $\textsf{Arbe-Gap}$ shown in \pref{alg:gap_estimation_balanced} is designed to identify a suitable candidate for the optimal policy and to estimate its gap. If such a policy that performs significantly better than any other policy emerges, the algorithm enters the second phase, $\textsf{Arbe-GapExploit}$ which further hones in on this policy by playing it most of the time while monitoring its regret in case the environment turns out to be adversarial after all. In the following, we describe both phases in more detail.

\subsection{First Phase: Candidate Policy Identification and Gap Estimation}

\begin{algorithm2e}[t]
\newcommand\mycommfont[1]{\textit{\textcolor{DarkBlue}{#1}}}
\SetCommentSty{mycommfont}
\textbf{Input:} failure probability $\delta$, timestep $t_0$, focus policy $\widehat{\pi}$, learners $\alg[s], \alg[s+1], \dots, \alg[M]$ \\% 
Set $\Pi_{M+1} = \Pi_M \backslash \{ \widehat{\pi}\}$ and $\alg[M+1]$ as a copy of $\alg[M]$ with policy class $\Pi_{M+1}$\\
Initialize base learners $\alg[s], \alg[s+1], \dots, \alg[M+1]$ with extended policy classes $\tilde \Pi_s, \tilde \Pi_{s+1}, \dots, \tilde \Pi_{M+1}$\\
Set sampling probabilities $\rho_i = \frac{R(\tilde \Pi_i)^{-2}}{\sum_{j=s}^{M+1} R(\tilde \Pi_j)^{-2}}$ for all $i \in \{s,\ldots, M+1\}$, and $\rho_i = 0$ for $i < s$\\
\For{round $t= t_0+1,t_0+2, \dots $}{
    Sample base learner index $b_t \sim \operatorname{Categorical}(\rho_1, \cdots, \rho_M)$\\
    Get context $x_t$ and
    compute $a_t^i \sim \pi_{t}^{i}(\cdot | x_t)$, the action each base learner $\alg[i]$ proposes for $x_t$\\
    Play action $a_t = a^{b_t}_t$ ( resolve linked actions if necessary) and receive reward $r_t(a_t,x_t)$.\\
   Update all base learners $\alg[i]$ with reward $\frac{\indicator{b_t = i} r_t(a_t,x_t)}{\rho_i}$\\ 
    \tcp{Balancing Elimination Test: $\alg[j]$ better than $\alg[i]$ for $i < j$?}
    \If{Equation~\ref{eqn:algorithm_misspecification_test_condition} holds between $\alg[i],\alg[j]$ for $s \leq i < j \leq M+1$}{
        restart algorithm by running \textsf{Arbe-Gap}$(\delta, t, \wh \pi, (\alg[i+1], \cdots, \alg[M]))$ 
    }
    \tcp{Gap Test: $\alg[M]$ better than $\alg[M+1]$?}
    Set $\textrm{W}(t_0, t) = \Ocal\left( \frac{R(\wt \Pi_M)}{\sqrt{(t - t_0)\rho_M}}\ln \frac{t}{\delta} \right)$ and $\wh \Delta_t = \frac{\tildecrew_M(t_0, t) - \tildecrew_{M+1}(t_0,t)}{t - t_0} - \textrm{W}(t_0, t)$\\
    \If{$\wh \Delta_t \geq 6\textrm{W}(t_0, t)$}{
    Start exploitation phase by running \textsf{Arbe-GapExploit} (pseudo-code in \pref{app:bestofboth}) with inputs $\wh \pi$,
  $t_{\mathrm{gap}} = t$ and $\wh \Delta_t$
    }
    
    
    
    
    \tcp{New Focus Policy Test}
    \If{there is a policy $ \pi \in \Pi_M \setminus \{ \wh \pi\}$ that has been selected in more than $\frac{3t}{4}$ of all $t$ rounds}{
    restart algorithm by running \textsf{Arbe-Gap}$(\delta, t, \pi, (\alg[s], \cdots, \alg[M]))$ 
}
}
\caption{\textsf{Arbe-Gap}$(\delta, t, \pi, (\alg[s], \dots, \alg[M])$}
\label{alg:gap_estimation_balanced}
\end{algorithm2e}


 The Gap Estimation Phase helps the learner identify a gap between the best policy and the rest if one exists (for example when the world is stochastic). When the world is stochastic with gap $\Delta$, this subroutine is designed to end after a number of timesteps that (ignoring logarithms and policy class complexities) scales with $\frac{1}{\Delta^2}$.  In this case, at the end of this phase the learner will be guaranteed to built a gap estimator $\widehat{\Delta}$ satisfying $\frac{\Delta}{2} \leq \widehat{\Delta} \leq \Delta$ with high probability. 
 The algorithm starts with an arbitrary guess $\widehat \pi$ for the optimal policy $\pi^*$ and plays $\alg[1], \cdots, \alg[M], \alg[M+1]$ such that $\alg[M+1]$ utilizes policy class $\Pi_{M+1} = \Pi_M \backslash \{\widehat{\pi}\}$. These algorithms are linked and played following a balancing schedule with probabilities $\rho_i = \frac{R(\widetilde \Pi_i)^{-2}}{\sum_{j=1}^{M+1} R(\widetilde\Pi_j)^{-2}}$. If algorithm $i$ is misspecified (see line 11 of Algorithm~\ref{alg:gap_estimation_balanced}), a new phase with a reduced set of learners is started. The balancing probabilities ensure the learner's adversarial regret scales with $R(\widetilde \Pi_{i_\star})$. 
 
The main challenge is to ensure $\widehat{\pi}$ converges to $\pi^*$ when the environment is stochastic. To achieve this we rely on the observation that in a stochastic world with gap $\Delta$, after sufficiently many timesteps (a time that up to logs and algorithm complexities scales with $1/\Delta^2$) any algorithm with a sublinear regret guarantee will have played $\pi^*$ more than $3/4$ of the time (see Appendix~\ref{app:bestofboth} for a proof). Thus line 15 of Algorithm~\ref{alg:gap_estimation_balanced} ensures that when the pseudo-regret across all phases is sublinear, $\widehat{\pi} $ will converge to $\pi^*$. Moreover, the number of restarts due to having found a new candidate policy $\widehat \pi$ grows at most logarithmically (see Appendix~\ref{app:bestofboth} for a proof). 


It can be shown these restarts degrades the performance of the model selection adversarial regret only by a $\sqrt{\log(t+1)}$ factor compared with \textsf{Arbe} so that $\regret(t) = \Ocal\left(  \frac{R^2(\widetilde{\Pi}_{i_\star})}{R(\widetilde{\Pi}_{1})}\sqrt{ i_\star M \log(t+1) t \ln \frac{t}{\delta} }   + M R(\widetilde{\Pi}_{i_\star}) \sqrt{ i_\star \log(t+1) t \ln\frac{t}{\delta} }     \right)$ for all $t \leq t_{\mathrm{gap}} := \text{last step in gap estimation}$. 






To build $\widehat{\Delta}$ we compare the performance of $\alg[M]$ (using policy class $\widetilde \Pi_M$) and $\alg[M+1]$ (with policy class $\Pi_M \backslash \{\widehat{\pi}\}$). If the average performance of $\alg[M+1]$ falls below a band of radius $\Theta\left(\frac{\U_{\rho_{M+1}}(\Pi_{M+1}, t)}{t}\right)$ \aldo{in algo this is $t-t_0$} below that of $\alg[M]$ (line 13 of Algorithm~\ref{alg:gap_estimation_balanced}), we build $\widehat \Delta$ by subtracting the lower and upper estimators of the optimal policy values for $\alg[M]$ and $\alg[M+1]$ (see line 14 in Algorithm~\ref{alg:gap_estimation_balanced}). This does not harm the model selection bounds.


If the environment is stochastic we shown that $t_{\mathrm{gap}} = \Ocal\left( \frac{\poly(R(\Pi_M) )   \log(1 / \delta) \log(1 /  \Delta)}{\Delta^2}\right)$. Moreover, the final policy $\widehat \pi = \pi^*$ and the gap estimator $\widehat \Delta$ satisfies $\frac{\Delta}{2} \leq \widehat \Delta \leq \Delta$ (see Appendix~\ref{app:bestofboth} for a formal statement). Applying the balanced regret upper bound to $t_\mathrm{gap}$ yields a poly-logarithimc regret guarantee of the form $ \pseudoregret(t) = \Ocal\left(  \frac{\poly(R(\Pi_M) )  \log(t/\delta) \sqrt{\log(1 / \delta) \log(1 /  \Delta)} }{\Delta}\right)$ for all $t\leq t_\mathrm{gap}$. 



\subsection{Second Phase: Exploitation}


Starting with a policy $\widehat \pi$ and a gap estimator $\widehat{\Delta}$, the learner will test the hypothesis `the environment is stochastic, $\widehat \pi $ is the optimal policy, and has a gap of order $\Theta(\widehat \Delta)$'. If any information arises contradicting this assumption we conclude the environment is adversarial. Since we are hoping to maintain a logarithmic rate in case the environment is stochastic, policy $\widehat{\Delta}$ must be played as often as possible, but without compromising the adversarial regret guarantee. 

The intuition driving our best of both worlds strategy is as follows. Policy $\widehat \pi$ will be played with probability roughly equal to $1-\frac{\tilde{c}}{\widehat{\Delta}^2 2^i}$ for some $i$, while an ensemble of balanced learners plays the policy class $\Pi_M \backslash \{ \widehat \pi \}$ with the remaining probability $\frac{\tilde{c}}{\widehat{\Delta}^2 2^i}$. Provided $1-\frac{\tilde{c}}{\widehat{\Delta}^22^i} \geq \frac{1}{2}$, the importance weighted estimator $\tildecrew_{\widehat{\pi}}(t)$ allows us to track the sum of pseudo-rewards of $\widehat \pi$ with $\sqrt{t}$ accuracy. Similarly, at time $t = 2^i$ the sum of the pseudo-rewards of the learners playing $\Pi_M \backslash \{ \widehat \pi \}$ can be tracked by $\tildecrew_{\Pi_M \backslash \{ \widehat{\pi} \} }(t)$ up to an $\approx c_1\widehat{\Delta} t$ accuracy. 

Using $h-$stability of the input learners operating over $\Pi_M \backslash \{ \widehat{\pi} \}$ we ensure these satisfy a pseudo-regret bound at time $t = 2^i$ w.r.t  the optimal policy in $\Pi_M \backslash \{ \widehat{\pi} \}$ of at most $c_1 \widehat{\Delta} t$. If $c_1 < 1/4$, the sum of errors between tracking and regret is upper bounded by $\frac{\widehat{\Delta} t}{4}$. We make use of a test that checks for that the sum of pseudo-rewards coming from the ensemble to be at least $\frac{\widehat{\Delta}t}{2}$ lower than the pseudo-rewards of $\widehat{\pi}$ but no more than $\frac{3\widehat{\Delta}t}{2}$ away. When the world is stochastic and $\widehat \pi$ equals $\pi^*$ this sandwich condition is satisfied. If this condition is ever violated, the environment must be adversarial. Moreover, if this condition holds, we would can ensure the pseudo-regret up to time $t$ is upper bounded by $\Ocal( \frac{ \tilde{c} \log(t)}{\widehat \Delta})$ and the adversarial regret has a $\sqrt{t}$ sublinear scaling. 

Our full algorithm can be found in Appendix~\ref{app:bestofboth}. It instantiates the intuition described above in the form of an epoch based algorithm that also incorporates a balancing test to ensure the adversarial regret satisfies a regret guarantee scaling with $R(\Pi_{i_\star})$. Additionally, our algorithm ensures the tracking and regret guarantees described above hold for all $t$ and not only for the epoch endpoint.











 
 
 



















